The Advice Complexity of a Class of Hard Online Problems

The advice complexity of an online problem is a measure of how much knowledge of the future an online algorithm needs in order to achieve a certain competitive ratio. Using advice complexity, we define the first online complexity class, AOC. The class includes independent set, vertex cover, dominating set, and several others as complete problems. AOC-complete problems are hard, since a single wrong answer by the online algorithm can have devastating consequences. For each of these problems, we show that $\log\left(1+(c-1)^{c-1}/c^{c}\right)n=\Theta (n/c)$ bits of advice are necessary and sufficient (up to an additive term of $O(\log n)$) to achieve a competitive ratio of $c$. The results are obtained by introducing a new string guessing problem related to those of Emek et al. (TCS 2011) and B\"ockenhauer et al. (TCS 2014). It turns out that this gives a powerful but easy-to-use method for providing both upper and lower bounds on the advice complexity of an entire class of online problems, the AOC-complete problems. Previous results of Halld\'orsson et al. (TCS 2002) on online independent set, in a related model, imply that the advice complexity of the problem is $\Theta (n/c)$. Our results improve on this by providing an exact formula for the higher-order term. For online disjoint path allocation, B\"ockenhauer et al. (ISAAC 2009) gave a lower bound of $\Omega (n/c)$ and an upper bound of $O((n\log c)/c)$ on the advice complexity. We improve on the upper bound by a factor of $\log c$. For the remaining problems, no bounds on their advice complexity were previously known.

==> apps_max.tex <==
\subsection{\Wmaxc maximization problems}
In this section, we consider two maximization problems which are \Wmaxc.
%\subsection{Online Independent Set}
\subsubsection{Online Independent Set.} The first maximization problem that we consider is \IS.

\begin{lemma}
\label{isupper}
\IS is in \Wmax.
\end{lemma}
\begin{proof}
Each request is a vertex along with the edges connecting it to previously requested vertices. The algorithm makes a binary choice for each request,
to include the vertex ($y_i=0$) or not ($y_i=1$). The feasible outputs are those that are independent sets. There exists a feasible output (taking no vertices).
The score of a feasible output is the number of vertices in it, and the score of an infeasible output is $-\infty$. Any subset of the vertices in an optimal solution is a feasible solution.
\end{proof}

\begin{lemma}
\label{iskh}
If there is a $c$-competitive algorithm reading $b$ bits for \IS, then there is a $c$-competitive algorithm reading $b + O(\log n)$ bits for \maxSk.
\end{lemma}

\begin{proof}
The proof is almost identical to the proof of Lemma \ref{vckh}.
Let \ALG be a $c$-competitive algorithm (with an additive constant of $\alpha$) for \IS reading at most $b$ bits of advice. We will define an algorithm \ALGp and an oracle \ORACLEp for \maxSk such that $\ALGp$ is $c$-competitive (with the same additive constant) and reads at most $b$ bits of advice.

As in Lemma \ref{vckh}, on input $x=x_1\ldots x_n$ to \IS, the algorithm \ALGp simulates \ALG on $G_x$ (from Definition~\ref{G}). This time, a vertex in $V_0$ is \emph{good} and a vertex in $V_1$ is \emph{bad}. Note that $V_0\cup\{v_n\}$ is a maximum independent set in $G_x$. Also, if \ALG accepts a bad vertex, $v_i$, then no further vertices $v_j$ (where $i<j\leq n$) can be accepted because of the edges $(v_i, v_j)$. Thus, \ALG accepts at most one bad vertex. Let $V_{\ALG}$ be the vertices accepted by \ALG. Since \ALG is $c$-competitive, $V_{\ALG}$ is an independent set satisfying $\ab{V_0}\leq \ab{V_0\cup\{v_n\}}\leq c\ab{V_{\ALG}}+\alpha$. We denote by $y$ the output computed by $\ALGp$. There are three cases to consider:

\emph{Case 1: All vertices accepted by $\ALG$ are good, that is $V_\ALG\subseteq V_0$.} In this case, \ALG answers $0$ in round $i$ if $v_i\in V_\ALG$ and $1$ otherwise. Clearly, $x \sq y$ and $\nz{x} = \ab{V_0}\leq c\ab{V_{\ALG}}+\alpha= c\nz{y}+\alpha$.
 
%If \ALG accepts a bad vertex, there are two subcases we need to take care of: Suppose that $V_\alg\subsetneq V_0$. Let $i$ be the lowest index such that $v_i\in V_1 \cap V_{\alg}$. Since there is an edge from $v_i$ to $v_j$ for all $i<j$, this means that $\{v_{i+1},\ldots , v_n\}\cap V_\alg =\emptyset$. In particular, $v_i$ is the only bad vertex chosen by $\ALG$.

\emph{Case 2a: \ALG accepts a bad vertex, $v_i$, and rejects a good vertex, $v_j$.} In this case, the oracle \ORACLEp writes the indices $i$ and $j$ in a self-delimiting way. \ALG simulates \ALGp as before, but answers $1$ in round $i$ and $0$ in round $j$. It follows that $x \sq y$ and $\nz{x}\leq c\nz{y}+\alpha$.

\emph{Case 2b: \ALG accepts a bad vertex, $v_i$, and all good vertices.} This implies that $V_\ALG$ is an independent set of size $\ab{V_0}+1$, which must be optimal. The oracle \ORACLEp writes the value of $i$ to the advice tape in a self-delimiting way. \ALG simulates \ALGp as before but answers $1$ in round $i$. It follows that $x \sq y$. Furthermore, $\nz{y}=\ab{V_{\ALG}}-1=\ab{V_0}=\nz{x}$, and hence the solution $y$ is optimal.

In order to simulate \ALG, the algorithm \ALGp needs to read at most $b$ bits of advice plus $O(\log n)$ bits of advice to specify the case and handle the cases where \ALG accepts a bad vertex. 
\end{proof}


% \begin{proof}
% The proof is almost identical to the proof of Lemma \ref{vckh}.
% Let \ALG be a $c$-competitive algorithm for \IS reading at most $b$ bits of advice. 
% We will define an algorithm \ALGp and an oracle \ORACLEp for \maxSk such that $\ALGp$ is $c$-competitive and reads at most $b$ bits of advice.
% Again, we will start by modifying $\ALG$ into a strictly $c$-competitive algorithm $\ALGs$ by using $O( \log n)$ additional advice bits.

% As in Lemma \ref{vckh}, on input $x=x_1\ldots x_n$ to \IS, the algorithm \ALGp simulates \ALGs on $G_x$ (from Definition~\ref{G}). 
% This time, a vertex is \emph{good} if it is in $V_0\cup\{v_n\}$ and \emph{bad} otherwise. 
% Note that $V_0\cup\{v_n\}$ is a maximum independent set in $G_x$.
% Also, if \ALG accepts a bad vertex, $v_i$, then no further vertices $v_j$ (where $i<j\leq n$) can be accepted because of the edges $(v_i, v_j)$. 
% Thus, \ALG accepts at most one bad vertex. 
% To construct $\ALGs$, $n$ is first written (with a self delimiting encoding) on the advice tape. Now, if $\ALG$ will take a bad vertex, the index of this is written.
% Finally, the indices of $\alpha+1$ good vertices that $\ALG$ does not take is written. Now, $\ALGs$ will simulate $\ALG$ but it will not take the bad vertex that $\ALG$ takes (if ones exists).
% Instead, it takes the $\alpha+1$ good vertices that $\ALG$ does not take (whose indices were written on tape). This means that $\ALGs$ gets at least $\alpha$ vertices more than $\ALG$, which makes
% it $c$-competitive. Note that if there does not exist $\alpha+1$ good vertices that were not taken, the indices of as many as possible is simply written. In this case, $\ALGs$ is strictly $1$-competitive.
 

% Let $V_{\ALGs}$ be the vertices accepted by \ALGs. 
% Now, \ALGp works by answering $0$ in round $i$ if $v_i\in V_\ALGs$ and $1$ otherwise in round 1 to $n-1$.
% Since \ALGp knows the value of $x_{i-1}$ at the beginning of round $i$ in \maxSk, \ALGp can use the advice to simulate \ALGs on $G_x$. 
% It will use one additional bit of advice to learn $x_n$ and guess correct there. We let $y$ denote the output string produced by $\ALGp$.
% If $x_n=0$, $\ALGs$ takes at least $\frac1{c}|V_0|$ vertices. Hence, $\ALGp$ guesses 0 at least $\frac1{c}|V_0|$. 
% If $x_n=1$, the maximum independent set has size $|V_0+1|$ (since it includes $x_n$). This means that $\ALGs$ gets an independent set of size at least $\frac1{c}(|V_0|+1)$.
% Since $\ALGp$ guessed 1 in round $x_n$ it answer 0 in at least $\frac1{c}(|V_0|+1)-1$ round, which is greater than $\frac1{c}|V_0|$.
% In both cases, we know that $\ALGp$ only guesses 0 when the correct answer is 0 since $\ALGs$ only takes good vertices. This shows that $\ALGp$ is a strictly $c$-competitive algorithm for \maxSk.
% It uses only $O( \log n)$ bits more than $\ALG$.
% \end{proof}
\begin{theorem}
\IS is \Wc.
\end{theorem}
\begin{proof}
This follows from Lemmas~\ref{isupper} and \ref{iskh} together with Theorem~\ref{kpacklow}.
\end{proof}


\subsubsection{Online Disjoint Path Allocation.}
In this section, we show that \DPA is \Wmaxc.
%In \DPA a path is given. Each request is a subpath given by the names of the two vertex endpoints.
%The subpath can either be taken or rejected.
%A solution is feasible if the paths that have been taken do not share any edges. In that case,
%the score is the number of paths. This problem is well studied. For a survey, see section~13.5 in \cite{BE98b}.


\begin{lemma}
\DPA is in \Wmax.
\end{lemma}

In Lemma~\ref{dpkh}, we use the same hard instance for \DPA as in \cite{A1} to get a lower bound on the advice complexity of \DPA.
\begin{lemma}
\label{dpkh}
If there is a $c$-competitive algorithm reading $b$ bits for \DPA, then there is a $c$-competitive algorithm reading $b + O(\log n)$ bits for \maxSk.
\end{lemma}
\begin{proof}
The proof is similar to the proof of Lemma \ref{iskh}. Let \ALG be a $c$-competitive algorithm for \DPA reading at most $b$ bits of advice. We will describe an algorithm \ALGp and an oracle \ORACLEp for \maxSk such that $\ALGp$ is $c$-competitive (with the same additive constant $\alpha$ as $\ALG$) and reads at most $b$ bits of advice. 

Let $x=x_1\ldots x_n$ be an input to \maxSk. We define an instance $I_x$ of \DPA with $L=2^{n}$ (that is, the number of vertices on the path is $2^{n}+1$).
In round $i$, $1 \leq i \leq n$, a path of length $2^{n-i}$ arrives.
For $2 \leq i \leq n$, the position of the path depends on $x_{i-1}$.
We define the request sequence inductively
(for an example, see Figure~\ref{fig:odpa}): 

\begin{figure}
\begin{align*}
&x=010\\
&L=8\\
&I_x = \langle (0,4), (4,6), (4,5) \rangle
\end{align*}
\caption{\label{fig:odpa}An example of the reduction used in the proof of Lemma~\ref{dpkh}. The request $(0,4)$ is good, since $x_1=0$, and $(4,6)$ is a bad request, since $x_2=1$.}
\end{figure}

In round $1$, the request $(u_1,v_1)$ arrives, where 
\begin{align*}
&u_1=0\\
&v_1=2^{n-1}
\end{align*}

In round $i$, $2\leq i\leq n$, the request $(u_i, v_i)$ arrives, where
\begin{align*}
&u_i=
  \begin{cases}
    u_{i-1}, & \text{if $x_{i-1}=1$}\\ 
    v_{i-1}, & \text{if $x_{i-1}=0$} 
  \end{cases}\\
&v_i=u_i+2^{n-i}
\end{align*}

We say that a request $r_i=(u_i, v_i)$ is \emph{good} if $x_i=0$ and \emph{bad} if $x_i=1$. If $r_i$ is good, then none of the later requests overlap with $r_i$. On the other hand, if $r_i$ is bad, then all later requests do overlap with $r_i$. In particular, if one accepts a single bad request, then no further requests can be accepted. An optimal solution is obtained if one accepts all good requests together with $r_n$.

The oracle \ORACLEp will provide \ALGp with the advice $\varphi$ read by \ALG when processing $I_x$. Since \ALG knows the value of $x_{i-1}$ at the beginning of round $i$ in \maxSk, \ALG can use the advice $\varphi$ to simulate \ALGp on $I_x$. If \ALG only accepts good requests, it is clear that \ALGp can compute an output $y$ such that $x \sq y$ and $\nz{x}\leq c\nz{y}+\alpha$. The case where \ALG accepts a bad request is handled by using at most $O(\log n)$ additional advice bits, exactly as in Lemma \ref{iskh}.
\end{proof}


\begin{theorem}
\DPA is \Wmaxc.
\end{theorem}
%We remark that our results shows that \DPA is \Wmaxc. For general graphs, there will be more than one way of connecting two vertices and so an algorithm has to do more than just making a binary choice. %, since there is exactly one way to connect two nodes in a tree, our \maxS algorithm can still be applied (and the lower bound for paths trivially also holds for trees).

%%% Local Variables:
%%% TeX-master: "Article.tex"
%%% End:




==> apps_min.tex <==
\subsection{\Wc Minimization Problems}\label{appmins}
In this section, we show that several online problems are \Wc, starting with \VC. See the introduction for the definition of the problems


\subsubsection{Online Vertex Cover.}

\begin{lemma} \label{VCupperlemma}
\VC is in \W.
\end{lemma}
\begin{proof}
We need to verify the conditions in Definition~\ref{wdef}. 

Recall that an input $\sigma= \langle r_1, \ldots, r_n \rangle$ for \VC is a sequence of requests, where each request is a vertex along with the edges connecting it to previously requested vertices. There is no dummy request at the end.
For each request, $r_i$, an algorithm makes a binary choice, $y_i$: It either includes the vertex into its solution ($y_i=1$) or not ($y_i=0$). 

The cost of an infeasible solution is $\infty$.
A solution $y=y_1 \ldots y_n$ for \VC is feasible if the vertices included in the solution form a vertex cover in the input graph. Clearly, there is always at least one feasible solution, since taking all the vertices will give a vertex cover. 

Thus, \VC has the right form.
Finally, we verify that conditions 1 and 2 are also satisfied: Condition 1 is satisfied since the cost of a feasible solution is the number of vertices in the solution and condition 2 is satisfied since a superset of a vertex cover is also a vertex cover. 
\end{proof}

We now show a hardness result for \VC. In our reduction, we make use of the following graph construction. The same construction will also be used later on for other problems. We remark that this graph construction is identical to the one used in \cite{Magnus} for showing lower bounds for \IS in the multi-solution model.

\begin{definition}[cf. \cite{Magnus}]
\label{G}
For any string $x=x_1\ldots x_n\in\{0,1\}^n$, define $G_x=(V,E)$ as follows:
\begin{align*}
V&=\{v_1,\ldots , v_n\},\\
E&=\{(v_i, v_j) \colon \text{$x_i=1$ and $i<j$}\}.
\end{align*} 
Furthermore, let $V_0=\{v_i \colon x_i=0\}$ and $V_1=\{v_i \colon x_i =1\}$.
\end{definition}

For a string $x\in\{0,1\}^n$, the graph $G_x$ from Definition~\ref{G} is a \emph{split graph}: The vertex set $V$ can be partitioned into $V_0$ and $V_1$ such that $V_0$ is an independent set of size $\nz{x}$ and $V_1$ is a clique of size $\no{x}$. 



\begin{figure}[h]
\centering
\begin{tikzpicture}[-,>=stealth',minimum size=0.75cm,node distance=2cm,
  thick,main node/.style={circle,fill=blue!20,minimum size=0.75cm,draw,font=\sffamily\Large\bfseries}]
\selectcolormodel{gray}

  \node[main node] (1) {{\small 0}};
  \node[main node] (2) [right=1 cm of 1] {{\small 1}};
  \node[main node] (3) [right=1 cm of 2] {{\small 1}};
  \node[main node] (4) [right=1 cm of 3] {{\small 0}};
  \node[main node] (5) [right=1 cm of 4] {{\small 1}};
  \node[main node] (6) [right=1 cm of 5] {{\small 0}};

  \path[every node/.style={font=\sffamily\small}]
	(2) edge (3)
	(2) edge [bend left] (4)
	(2) edge [bend left] (5)
	(2) edge [bend left] (6)
	(3) edge (4)
	(3) edge [bend right] (5)
	(3) edge [bend right] (6)
	(5) edge (6)

	;
\end{tikzpicture}
\caption{$G_{011010}$}
\end{figure}

\begin{lemma}
\label{vckh}
If there is a $c$-competitive algorithm reading $\advice$ bits for \VC, then there is a $c$-competitive algorithm reading $\advice + O(\log n)$ bits for \minSk.
\end{lemma}
\begin{proof}
Let $\ALG$ be a $c$-competitive algorithm for \VC reading at most $\advice$ bits of advice. By definition, there exists a constant $\alpha$ such that $\ALG(\sigma)\leq c\cdot\OPT(\sigma)+\alpha$ for any input sequence $\sigma$. We will define an algorithm, $\ALGp$, and an oracle, \ORACLEp, for \minSk such that $\ALGp$ is $c$-competitive (with the same additive constant) and reads at most $\advice+ O(\log n)$ bits of advice.

For $x=x_1\ldots x_n$ an input string to \minSk, consider the input instance to \VC $G_x=(V,E)$ defined in Definition~\ref{G} where the vertices are requested in the order $\langle v_1, \ldots, v_n\rangle$. We say that a vertex in $V_0$ is \emph{bad} and that a vertex in $V_1$ is \emph{good}. Note that $V_1\setminus\{v_n\}$ is a minimum vertex cover of $G_x$. Also, if an algorithm rejects a good vertex $v_i$, then it must accept all later vertices $v_j$ (where $i<j\leq n$) in order to cover the edges $(v_i, v_j)$. In particular, since the good vertices form a clique, no algorithm can reject more than one good vertex.

Let $\varphi$ be the advice read by $\ALG$, and let $V_{\ALG}$ be the vertices chosen by $\ALG$. Since $\ALG$ is $c$-competitive, we know that $V_{\ALG}$ must be a vertex cover of size at most $c\ab{V_1\setminus\{v_n\}}+\alpha\leq c\ab{V_1}+\alpha$. 

We now define $\ALGp$ and $\ORACLEp$. As usual, $y$ denotes the output computed by $\ALGp$. We consider three cases. The first two bits of the advice tape will be used to tell \ALGp which one of the three cases we are in. 

\emph{Case 1: $\ALG$ accepts all good vertices in $G_x$, i.e., $V_1\subseteq V_\ALG$.}
 The oracle \ORACLEp writes the advice $\varphi$ to the advice tape. When $\ALGp$ receives request $i$, it considers what $\ALG$ does when the vertex $v_i$ in $G_x$ is revealed: \ALGp answers $1$ if \ALG accepts $v_i$ and $0$ otherwise. Note that it is possible for $\ALGp$ to simulate $\ALG$ since, at the beginning of round $i$, $\ALGp$ knows $x_1\ldots x_{i-1}$. In particular, $\ALGp$ knows which edges to reveal to $\ALG$ along with the vertex $v_i$ in $G_x$. Together with access to the advice $\varphi$ read by $\ALG$, this allows $\ALGp$ to simulate $\ALG$. Since $V_1\subseteq V_\ALG$, we get that $x\sq y$. Furthermore, since $\ab{V_\ALG}\leq c\ab{V_1}+\alpha$, we also get that $\no{y}\leq c\no{x}+\alpha$.

%Suppose now that \ALG rejects a good vertex. Recall that this implies that \ALG must accept all later vertices.

%\emph{Case 2: \ALG rejects a good vertex, $v_i$.} Recall that $v_i$ must be the only good vertex rejected by $\ALG$. In this case, the oracle \ORACLEp first writes a 1 to the advice tape, and then the index $i$ in a self-delimiting way, followed by $\varphi$. $\ALGp$ simulates $\ALG$ as before and answers accordingly, except that it answers $1$ in round $i$. This ensures that $x\sq y$. Furthermore, $\no{y}=\ab{V_\ALG}+1\leq c\ab{V_1}+\alpha+1= c\no{x}+(\alpha+1)$.

\emph{Case 2a: \ALG rejects a good vertex, $v_i$, and accepts a bad vertex, $v_j$.} In this case, the oracle \ORACLEp writes the indices of $i$ and $j$ in a self-delimiting way, followed by $\varphi$, to the advice tape. $\ALGp$ simulates $\ALG$ as before and answers accordingly, except that it answers $1$ in round $i$ and $0$ in round $j$. This ensures that $x\sq y$. Furthermore, $\no{y}=\ab{V_\ALG}\leq c\ab{V_1}+\alpha= c\no{x}+\alpha$.

\emph{Case 2b: \ALG rejects a good vertex, $v_i$, and all bad vertices.} In this case, $V_{\ALG}=V_1\setminus\{v_i\}$. The oracle \ORACLEp writes 
the value of $i$ to the advice tape in a self-delimiting way, followed by $\varphi$. Again, \ALGp simulates \ALG, but it answers $1$ in round $i$. 
Thus, $x=y$, meaning that $x \sq y$ and $y$ is optimal.

In all cases, $\ALGp$ computes an output $y$ such that $x\sq y$ and $\no{y}\leq c\no{x}+\alpha$. 
Since $\ab{\varphi}\leq \advice$, the maximum number of bits read by $\ALGp$ is $\advice+O(\log n)+2=\advice+O(\log n)$.
\end{proof}


\begin{theorem}
\VC is \Wc.
\end{theorem}
\begin{proof}
By Lemma~\ref{VCupperlemma}, \VC is in \W. Combining Lemma~\ref{vckh} and Theorem~\ref{lminknown} shows that a $c$-competitive algorithm for \VC must read at least $B(n,c)-O(\log n)$ bits of advice. Thus, \VC is \Wc.
\end{proof}


%It is useful to think of \VC being in \sgeasymin because a superset of a feasible solution is still a feasible. In fact, using the same model of requesting vertices in a graph,
%you can replace the constaint that the chosen vertices have to form a vertex cover with any other constraint with the property that a superset of a feasible solution is still feasible.
%This means that several natural problems are in fact in \sgeasymin. The following problem illustrates this.

\subsubsection{Online Cycle Finding.}
Most of the graph problems that we prove to be \Wc are, in their offline versions, $\mathsf{NP}$-complete. However, in this section, we show that \CF is also \Wc. The offline version of this problem is very simple and can easily be solved in polynomial time.

%another very simple problem, which can be solved in polynomial time offline.
%In \CF, the goal is to select the smallest number of vertices of a simple graph, $G$, such that the graph induced by them contains at least one cycle (we assume that $G$ has a cycle). Note that at least three vertices are needed to form a cycle.
%Exactly as in Online Vertex Cover, the vertices of $G$ are revealed one by one and for each one. The algorithm can take a vertex or reject it.
%As in vertex cover, when a vertex is revealed, it is also revealed which previous vertices it is adjacent to.
%When all vertices have been revealed, the cost of the output is defined in the following way:

%If the graph induced by the taken vertices contanis a cycle, the cost of it is the number of vertices included in the output.
%Otherwise, the cost is said to be $\infty$.

\begin{lemma} \label{cfub}
\CF is in \W.
\end{lemma}
This and the following proofs of membership of \W have been omitted. They are almost identical to the proof of Lemma~\ref{VCupperlemma}.

In order to show that \CF is \Wminc, we will make use of the following graph.

\begin{definition}
\label{H}
For a string $x=x_1\ldots x_n\in\{0,1\}^n$ define $f(x_i)$ to be the largest $j<i$ such that $x_j=1$.
Note that this may not always be defined. We let $\textsc{max}$ be the largest $i$ such that $x_i=1$. Similarly, we let $\textsc{min}$ be the smallest $i$ such that $x_i=1$.
We now define the graph $H_x=(V,E)$:
\begin{align*}
V&=\{v_1,\ldots , v_n\},\\
E&=\{(v_j, v_i) \colon f(x_i)=j\} \cup \{ (v_{\textsc{min}}, v_\textsc{max})\}.
\end{align*} 
Furthermore, let $V_0=\{v_i \colon x_i=0\}$ and $V_1=\{v_i \colon x_i =1\}$.
\end{definition}

\begin{figure}[h]
\centering
\begin{tikzpicture}[-,=stealth',minimum size=0.75cm,node distance=2cm,
  thick,main node/.style={circle,fill=blue!20,minimum size=0.75cm,draw,font=\sffamily\Large\bfseries}]
\selectcolormodel{gray}
  \node[main node] (1) {{\small 0}};
  \node[main node] (2) [right=1 cm of 1] {{\small 1}};
  \node[main node] (3) [right=1 cm of 2] {{\small 0}};
  \node[main node] (4) [right=1 cm of 3] {{\small 0}};
  \node[main node] (5) [right=1 cm of 4] {{\small 1}};
  \node[main node] (6) [right=1 cm of 5] {{\small 0}};
  \node[main node] (7) [right=1 cm of 6] {{\small 1}};

  \path[every node/.style={font=\sffamily\small}]
	(2) edge (3)
	(2) edge [bend left] (4)
	(2) edge [bend left] (5)
	(2) edge [bend right] (7)
	(5) edge (6)
	(5) edge [bend left] (7)

	;
\end{tikzpicture}
\caption{$H_{0100101}$}
\end{figure}

\begin{lemma}
\label{cfkh}
If there is a $c$-competitive algorithm reading $\advice$ bits for \CF, then there is a $c$-competitive algorithm reading $\advice + O(\log n)$ bits for \minSk.
\end{lemma}
\begin{proof}
Let $\ALG$ be a $c$-competitive algorithm (with an additive constant $\alpha$) for \CF reading at most $\advice$ bits of advice. We will define an algorithm $\ALGp$ and an oracle \ORACLEp for \minSk such that $\ALGp$ is $c$-competitive (with the same additive constant) and reads at most $\advice+ O(\log n)$ bits of advice.

Let $x=x_1\ldots x_n$ be an input string to \minSk. The oracle \ORACLEp first writes one bit of advice to indicate if $\no{x}\leq 2$. If this is the case, \ORACLEp writes (in a self-delimiting way) the index of these at most two $1$s to the advice tape. This can be done using $O(\log n)$ bits and clearly allows \ALGp to be strictly $1$-competitive. In the rest of the proof, we will assume that there are at least three 1s in $x$.

Consider the input instance to \CF, $H_x=(V,E)$, defined in Definition~\ref{H}, where the vertices are requested in the order $\langle v_1, \ldots, v_n\rangle$. Note that the vertices $V_1$ form the only cycle in $H_x$. Thus, if an algorithm rejects a vertex from $V_1$, the subgraph induced by the vertices accepted by the algorithm cannot contain a cycle.

Let $\varphi$ be the advice read by $\ALG$, and let $V_{\ALG}$ be the vertices chosen by $\ALG$, when the $n$ vertices of $H_x$ are revealed. Since $\ALG$ is $c$-competitive, we know that $\ab{V_{\ALG}}\leq c\ab{V_1}+\alpha$.

We now define $\ALGp$. As usual, $y$ denotes the output computed by $\ALGp$. Since $\ALG$ is $c$-competitive, it must hold that $V_1\subseteq V_\ALG$. The oracle \ORACLEp writes the advice $\varphi$ to the advice tape. When $\ALGp$ receives request $i$ at the beginning of round $i$ in \minSk, it considers what $\ALG$ does when the vertex $v_i$ in $H_x$ is revealed: \ALGp answers $1$ if \ALG accepts $v_i$ and $0$ otherwise. Note that it is possible for $\ALGp$ to simulate $\ALG$ since, at the beginning of round $i$, $\ALGp$ knows $x_1\ldots x_{i-1}$. In particular, $\ALGp$ knows which edges were revealed to $\ALG$ along with the vertex $v_i$ in $H_x$. Note, however, that in order to simulate the edge from $v_{\textsc{min}}$ to $v_{\textsc{max}}$, $\ALG$ needs to know when $v_{\textsc{max}}$ is being revealed.
This can be achieved using $O(\log n)$ additional advice bits.

 Together with access to the advice $\varphi$ read by $\ALG$, this allows $\ALGp$ to simulate $\ALG$. Since $V_1\subseteq V_\ALG$, we get that $x\sq y$. Furthermore, since $\ab{V_\ALG}\leq c\ab{V_1}+\alpha$, we also get that $\no{y}\leq c\no{x}+\alpha$.
\end{proof}

\begin{theorem}
\CF is \Wcomplete
\end{theorem}
\begin{proof}
This follows from Lemmas~\ref{cfub} and \ref{cfkh} together with Theorem~\ref{lminknown}.
\end{proof}

\subsubsection{Online Dominating Set.}
In this section, we show that \DS is also \Wminc. We do not require that the vertices picked by the online algorithm form a dominating set at all times. We only require that the solution produced by the algorithm is a dominating set when the request sequence ends. Of course, this makes a difference only because we consider online algorithms with advice. %It is possible that the algorithm knows that it will get a chance later on to dominate some currently undominated vertex. 
For \VC, this issue did not arise, since it is not possible to end up with a vertex cover without maintaining a vertex cover at all times. Thus, in this aspect, \DS is more similar to \CF.

\begin{lemma}
\label{dsup}
\DS in in \Wmin.
\end{lemma}
In order to show that \DS is \Wminc, we use the following construction. 

\begin{definition}
\label{K}
For a string $x=x_1 \ldots x_n$ such that $\no{x}\geq 1$, define $\textsc{max}$ to be the largest $i$ such that $x_i=1$ and define $K_x=(V,E)$ as follows:
\begin{align*}
V&=\{v_1,\ldots , v_n\},\\
E&=\{(v_i, v_{\textsc{max}}) \colon x_i=0\}.
\end{align*} 
Furthermore, let $V_0=\{v_i \colon x_i=0\}$ and $V_1=\{v_i \colon x_i =1\}$.
\end{definition}

Note that $V_1$ is a smallest dominating set in $K_x$ and that any dominating set is either a superset of $V_1$ or equal to $V \setminus \{v_{\textsc{max}}\}$. 
We now give a lower bound on the advice complexity of \DS. Interestingly, it is possible to do this by making a reduction from \minSu (instead of \minSk) to \DS.

\begin{lemma} \label{dshard}
If there is a $c$-competitive algorithm for \DS reading $\advice$ bits of advice, then there is a $c$-competitive algorithm reading $\advice+ O(\log n)$ bits
of advice for \minSu.
\end{lemma}
\begin{proof}
Let $\ALG$ be a $c$-competitive algorithm (with an additive constant of $\alpha$) for \DS reading at most $\advice$ bits of advice. We will define an algorithm $\ALGp$ and an oracle \ORACLEp for \minSu such that $\ALGp$ is $c$-competitive (with the same additive constant) and reads at most $\advice+ O(\log n)$ bits of advice.

Let $x=x_1\ldots x_n$ be an input string to \minSu. The oracle \ORACLEp first writes one bit of advice to indicate if $\no{x}=0$. If this is the case, \ALGp answers 0 in each round. In the rest of the proof, we will assume that $\no{x}\geq 1$.

Consider the input instance to \DS, $K_x=(V,E)$, defined in Definition~\ref{K}, where the vertices are requested in the order $\langle v_1, \ldots, v_n \rangle$. Note that $V_1$ is the smallest dominating set in $K_x$.
Let $\varphi$ be the advice read by $\ALG$, and let $V_{\ALG}$ be the vertices chosen by $\ALG$, when the $n$ vertices of $K_x$ are revealed. Since $\ALG$ is $c$-competitive, we know that $V_{\ALG}$ is a dominating set of size $\ab{V_{\ALG}}\leq c\ab{V_1}+\alpha$. 

We now define $\ALGp$ and $\ORACLEp$. 
The second bit of the advice tape will be used to let \ALGp distinguish the two cases described below.
Note that the only vertex from $V_1$ that can be rejected by a $c$-competitive algorithm is $v_{\textsc{max}}$, and nothing can be rejected when $V_1=V$. Hence the two cases are exhaustive.

{\em Case 1: \ALG accepts all vertices in $V_1$.}
The oracle \ORACLEp writes the value of $\textsc{max}$ in a self-delimiting way. This requires $O(\log n)$ bits. Furthermore, \ORACLEp writes $\varphi$ to the advice tape.
Now, \ALGp learns $\varphi$ and $\textsc{max}$ and works as follows: In round $i\leq \textsc{max}-1$, \ALGp answers 1 if $\ALG$ accepts the vertex $v_i$ and 0 otherwise. Note that \ALGp knows that no edges are revealed to \ALG in the first $\textsc{max}-1$ rounds. Thus, \ALGp can compute the answer produced by \ALG in these rounds from $\varphi$ alone. In round $\textsc{max}$, \ALGp answers $1$. In rounds $\textsc{max}+1,\ldots , n$, the algorithm \ALGp always answers $0$. 

{\em Case 2: \ALG rejects $v_{\textsc{max}}$.}
In order to dominate $v_{\textsc{max}}$, \ALG must accept a vertex $v_i \in V_0$.
The oracle \ORACLEp writes the values of $\textsc{max}$ and $i$ in a self-delimiting way, followed by $\varphi$, to the advice tape.
\ALGp behaves as in Case 1, except that it answers 0 in round $i$.

In both cases, $x\sq y$ and $\no{y}\leq \ab{V_{\ALG}}\leq c\ab{V_{1}}+\alpha = c\no{x}+\alpha$. Furthermore, \ALGp reads $\advice + O(\log n)$ bits of advice.
\end{proof}


\begin{theorem}
\DS is \Wcomplete
\end{theorem}
\begin{proof}
This follows from Lemmas~\ref{dsup} and \ref{dshard} together with Theorem~\ref{lminknown}.
\end{proof}



\subsubsection{Online Set Cover.}
We study a version of \SC in which the universe is known from the beginning and the sets arrive online. 
Note that this problem is very different from the set cover problem studied in \cite{setcover, Asetcover}, where the elements (and not the sets) arrive online. 

\begin{lemma} \label{scw}
\SC is in \W
\end{lemma}

\begin{lemma} \label{schard}
If there is a $c$-competitive algorithm for \SC reading $\advice$ bits of advice, then there
is a $c$-competitive algorithm reading $\advice + O(\log n)$ bits of advice for \minSu.
\end{lemma}
\begin{proof}
Let $x=x_1\ldots x_n$ be an input string to \minSu with $\no{x}\geq 1$, and define {\sc max} as in Definition~\ref{K}. We define an instance of \SC as follows.
The universe is $[n]=\{1,\ldots , n\}$ and there are $n$ requests. For $i \neq \textsc{max}$, request $i$ is just the singleton $\{i\}$. Request $\textsc{max}$ is the set $\{\textsc{max}\}\cup S_0$, where $S_0=\{i : x_i=0\}$.

Using these instances of \SC and the same arguments as in Lemma~\ref{dshard} proves the theorem.
Note that for \SC, only Case 1 of Lemma~\ref{dshard} is relevant, since a $c$-competitive algorithm for this problem will accept all requests $i \not\in S_0$.
\end{proof}

\begin{theorem}
\SC is \Wc
\end{theorem}
\begin{proof}
This follows from Lemmas~\ref{scw} and \ref{schard} together with Theorem~\ref{lminknown}.
\end{proof}


%%% Local Variables:
%%% TeX-master: "Article.tex"
%%% End:

